Presentation Proposal: Towards Efficient Data-flow Test Data Generation Using KLEE

Dataflow coverage, one of the white-box testing criteria, focuses on the relations between variable definitions and their uses.Several empirical studies have proved data-flow testing is more effective than control-flow testing. However, data-flow testing still cannot find its adoption in practice, due to the lack of effective tool support. To this end, we propose a guided symbolic execution approach to efficiently search for program paths to satisfy data-flow coverage criteria. We implemented this approach on KLEE and evaluated with 30 program subjects which are constructed by the subjects used in previous data-flow testing literature, SIR, SV-COMP benchmarks. Moreover, we are planning to integrate the data-flow testing technique into the new proposed symbolic execution engine, SmartUnit, which is a cloud-based unit testing service for industrial software, supporting coverage-based testing. It has successfully helped several well-known corporations and institutions in China to adopt coverage-based testing in practice, totally tested more than one million lines of real code from industry.

==> KLEE workshop/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-sigconf.tex \



PDF = ${SAMPLES:%.tex=%.pdf}

all:  ${PDF} clean


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-sigconf.pdf : introduction.tex \
					 approach_and_implementation.tex \
					 evaluation_and_discussion.tex \
					 related_work.tex \
					 conclusion.tex 



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	# $(RM) $(PACKAGE).cls *.log *.aux \
	# *.cfg *.glo *.idx *.toc \
	# *.ilg *.ind *.out *.lof \
	# *.lot *.bbl *.blg *.gls *.cut *.hd \
	# *.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf


==> KLEE workshop/approach_and_implementation.tex <==
\section{Approach and Implementation}

\subsection{Approach}
According to the Herman's definition~\cite{herman1976data}, a \emph{def-use pair} exists when there is at least one program \emph{path} from the \emph{definition} of variable to the \emph{use}
where there are no redefinitions between \emph{definition} and \emph{use}. For a \emph{def-use pair}, if there is an input \emph{t} that induces an execution path passing through \emph{definition} and then \emph{use} with no intermediate 
redefinitions of \emph{x} between \emph{definition} and \emph{use}, the input \emph{t} satisfies the \emph{def-use pair}. The requirement to cover all \emph{def-use pairs} at least once is called \emph{def-use coverage criterion}.

\begin{figure}
    \includegraphics[width=0.4\textwidth]{Figs/data-flow_testing_process.png}
    \caption{The basic process of data-flow testing.}
    \label{fig:process}
\end{figure}

Figure.~\ref{fig:process} shows the basic process of data-flow testing. 
For an input program, we perform static analysis to get a set of def-use pairs.
At each time, the test generator selects a pair as the target to find a test input covering the pair.
If the generator successfully generates the test input covering the pair, the test input will be put in the test suite, otherwise, the pair is regarded as the unsatisfiable pair within the given testing time.

To achieve efficient data-flow testing, we designed a \emph{cut-points guided search algorithm} to enhance symbolic execution~\cite{su2015combining}. The key idea of the strategy is to reduce unnecessary path exploration and provide more guidance during execution.
There are three key elements used to optimize the strategy: \emph{Cut Points}, \emph{Instruction Distance} and \emph{Redefinition Pruning}.
(1) \emph{Cut Points} is a sequence of control points that must be traversed through by any path that could cover the target pair. 
These cut points are used as intermediate goals during the search to narrow down the exploration space of symbolic execution.
(2) \emph{Instruction Distance} is the distance between currently executed instruction and target instruction in the control flow graph. 
The execution state which has shorter instruction distance toward the goal can reach it more easily.
(3) \emph{Redefinition Pruning} is the strategy that gives lower priority to the execution states which have the redefinitions on paths.
According to the definition of \emph{covering def-use pair}, the path which has redefinitions between \emph{definition} and \emph{use} is invalid.
Pruning the potential invalid paths can avoid useless explorations.

\subsection{Implementation}
Our implementation follows the basic data-flow testing process. 
In the data-flow analysis phase,
the input program is analyzed by CIL~\cite{necula2002cil} tool which is an infrastructure for C program analysis and transformation to identify the def-use pairs, cut points, and static program information. 
We use CIL instead of LLVM because we intend to analyze def-use pairs from source-level instead of bytecode level (LLVM IR).
The test data generation and coverage computation phase are implemented on KLEE. 

In detail, we implemented a searcher class in KLEE to apply our cut-points guided search strategy. 
Furthermore, we constructed a data-flow information table in KLEE to supply some extra data-flow information such as redefinitions and cut points during execution. 
A coverage checker and a redefinition checker are also implemented in KLEE based on the process tree. 
If an execution state reaches the use through the definition without any redefinition on the path, 
the coverage checker identifies that it has covered the pair.
Then the execution state generates the test case satisfying the pair.

==> KLEE workshop/conclusion.tex <==
\section{conclusion}

In this presentation, we propose an efficient data-flow test data generation algorithm implemented on KLEE and evaluated on a diverse set of program subjects.
It enables efficient and effective data-flow testing and helps several corporations and institutions to adopt data-flow testing in practice.

==> KLEE workshop/evaluation_and_discussion.tex <==
\section{evaluation and discussion} 

Although data-flow testing has been investigated for a long time, there are still no standard benchmark programs for evaluating data-flow testing techniques.
To set up a fair evaluation basis, we constructed our benchmarks as follows: (1) We conducted a survey on previous data-flow testing literature~\cite{su2017survey}. 
After excluding the subjects that are not available, not written in C language and simple laboratory programs, 
we finally got 7 subjects. (2) The benchmark included 7 Simens subjects from SIR which are widely used in the experiments of program analysis and software testing. 
(3) We further enriched the repository with 16 distinct subjects from SV-COMP which is used in the competition for software verification. We chose two groups of subjects in SV-COMP benchmark, \textsf{ntdriver group} (with 6 subjects) and \textsf{ssh} group (with 10 subjects).
The code and pair scale of each categories are showed in Table.~\ref{table:tools}.


\begin{table}[!t]
\scriptsize
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
\caption{Evaluation Statistic of Data-flow Testing via KLEE}
\label{table:tools}
\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
\begin{tabular}{|c||c|c|c|c|c|c|c|}
\hline
Subjects &\#Sub &\#LOC &\#DU pair &\multicolumn{2}{c|}{Average Coverage} &\multicolumn{2}{c|}{\makecell{Median Time \\ (s/pair)}}\\
\hline
& & & &KLEE &CPA &KLEE &CPA \\
Previous Literature &7 &449 &346  &60\% &72\% &0.1 &4.3\\ %0.23s
SIR &7 &2,687 &1,409 &57\% &60\% &0.7 &10.1\\
SV-COMP \textsf{(ntdriver)} &6 &7,266 &2,691 &75\% &51\% &1.5 &5\\
SV-COMP \textsf{(ssh)} &10 &5,249 &18,347 &29\% &31\% &18 &5.7\\
\hline
\end{tabular}
\end{table}
Table.~\ref{table:tools} gives an overview of our evaluation. It shows the data-flow coverage (The ratio between the number of covered pairs and the total number of pairs) and median test time of KLEE and CPAchecker approach~\cite{su2015combining}.
From Table~\ref{table:tools}, we can find that KLEE can easily achieve nearly 60\% of data-flow coverage within less than 1 second for each pair in the subjects from previous literature and SIR subjects.
Comparing with the model-checking approach implemented on CPAchecker, it spends less time and achieves the similar coverage in most of the subjects.
We found the longer median time in SV-COMP \textsf{ssh} benchmark is caused by the its complexity, which have complicate loops.
The existence of a large number of infeasible pairs is also a obstacle for applying symbolic execution in practice, since it will waste much time on useless exploration.
To solve this problem, we use model-checking to filter out the infeasible pairs in order to keep symbolic execution away from useless explorations.

==> KLEE workshop/evaluation_setup.tex <==
\section{Evaluation Setup}
\subsection{Research Questions}
To achieve the goal, we intend to set up some research questions which can guide our evaluation. 
The research questions are described as follows:
\begin{itemize}
  \item \textbf{\textit{RQ1}}: How about the performance of automated unit test generation framework SmartUnit in both commercial embedded software and open-source database software?
        In this paper, we use statement coverage, branch coverage, and MC/DC as evaluation indicators.
  \item \textbf{\textit{RQ2}}: What factors make dynamic symbolic execution get low coverage? 
  \item \textbf{\textit{RQ3}}: Can SmartUnit find the potential runtime exceptions in real-world software?
  \item \textbf{\textit{RQ4}}: What is the difference in terms of time, cost and quality between automatically generated test cases and manually written test cases? 
\end{itemize}

We package the the code under test and submit them to the SmartUnit cloud platform. SmartUnit can start dynamic symbolic execution automatically.
After the execution, a series of packaged .tcf files (the test cases) for the codes can be downloaded from the platform. 
We import the test cases into Testbed to get the coverage and detect the runtime error.
Testbed will generate a detailed testing report after running the automatically generated unit test cases.
Statement, branch and MC/DC coverage, runtime errors, and static errors are provided by the report.

The statement, branch and MC/DC coverage of each function will be recorded as the performance indicator for \textit{RQ1}. 
We turn our attention to the functions which gets low coverage in the three coverage criteria above, to answer \textit{RQ2}.
The runtime errors will be classified into a several of categories, so that we can obtain some insights from them, in \textit{RQ3}.
It's impossible to manually write test cases for all of the benchmark, because of the large scale of the software in the benchmark. 
We will select some representative codes to answer \textit{RQ4}.

\subsection{Benchmark}
This paper selects two kinds of C program benchmarks for SmartUnit: commercial embedded software and open-source database software.
Table ~\ref{table:benchmark} gives the list of benchmarks for the evaluation. Due to the confidentiality agreement, 
we hide the commercial software names in this paper.

\begin{table}[!t]
\footnotesize
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
\caption{Subjects of Evaluation Benchmark Repository.}
\label{table:benchmark}
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
\begin{tabular}{|c||c|c|c|}
\hline
Subject &\# Files &\# Functions &\# LOC\\
\hline
\hline
aerospace software &8 &54 &3,769\\
automotive software &4 &330 &31,760\\
subway signal software &108 &874 &37,506\\
SQLite &2 &2046 &126,691\\
PostgreSQL &906 &6105 &279,809\\
\hline
\hline
Total &1028 &9,409 &479,535\\
\hline
\end{tabular}
\end{table}

\textbf{The commercial embedded software} comes from aerospace, automotive, subway signal companies.
SmartUnit has tested millions of code from commercial embedded software. For example, 
in the aerospace company, SmartUnit tested more than 100,000 LOC. Over 70\% functions have achieved
more than 90\% statement coverage. In order to intensively study, we selected three benchmarks from the different areas to get a variety of characteristics. All of them come from real-world industrial code.

\textbf{The open-source database software} used in this paper are \textit{SQLite}\footnote{https://www.sqlite.org/} and \textit{PostgreSQL}\footnote{https://www.postgresql.org/}. 
Due to security demand of the commercial embedded software, we mainly use the open-source database software to explain.
We chose SQLite because it is an embedded SQL database engine, usually used in embedded software systems. 
It is a good sample for us to find some insights when using SmartUnit on the embedded system, which has nearly 200,000 LOC. 
The PostgreSQL is a representative object-relation database system, usually used as the enterprise-class database.
We chose PostgreSQL as a benchmark in order to evaluate performance and expandability of SmartUnit on the enterprise-class system.

For each subject, we put all of the .c and .h files into one folder to make it easier for Smartunit to get the relied header files for under test functions.
We divided each subject into an independent .zip package so that we can calculate coverage respectively.


\subsection{Evaluation Environment}
SmartUnit was run on a virtual machine with three processors and 3GB memory, CentOS operating system.

Testbed was run on a virtual machine with two processors(2.70GHz Intel(R) Core(TM) i5-2500S CPU) and 1GB memory, 
32bit Microsoft Windows XP Professional Service Pack 3 operating system.






==> KLEE workshop/framework_implementation.tex <==
\section{Framework Implementation}
\subsection{Framework Architecture}
Figure.~\ref{fig:backend} shows the core framework of SmartUnit.
\begin{figure}
    \includegraphics[width=0.3\textwidth]{Figs/backend.pdf}
    \caption{The architecture of SmartUnit.}
    \label{fig:backend}
\end{figure}
The basic process of generating test cases in our approach is as follows:

SmartUnit accepts the .c and .h files as its input. To deal with macros and make sure some external symbols can be introduced into the source file, we use \textit{libclang}\footnote{http://clang.llvm.org/doxygen/group\_\_CINDEX.html} as preprocessor to generate processed.c file. Then libclang is also used to parse the processed file to generate the AST (abstract syntax tree).

We establish the CFG (control flow graph) model based on the abstract syntax tree generated in the previous step, which consists control flow graph of the file being proceeded, in which type information of variables, expressions, functions and so on is stored to be used in further analysis. Each node in control flow graph represents a statement block in the source code. A sequential node, which contains exactly one incoming edge and one outgoing edge, contains no branch, meanwhile a branch node, which contains one incoming edge and more than one outgoing edge every of which shows a condition of a branch, is a statement block that contains conditional statements, such as if-else statement, while statement, switch statement \etc. 

\subsection{Executor Module}
Executor module consists of the memory model, executor, and searcher. This part mainly processes the CFG model given by former steps.

\subsubsection{Executor}
Executor executes the statement expressions in the current node and drives the searcher to select next edge to explore. The executor does not really execute the C statements, it actually transforms the C statement into blocks, declarations or expressions structures that are stored inside SmartUnit. The executor updates information in CFG model and adds constraints to a path, after gathering them from the node statement. After the executor reaches the end node, it collects all constraints on the path, and solves them by constraint solver such as Z3 prover.

\subsubsection{Searcher and Search Strategies}
To perform the search on control flow graph, we put forward a new search strategy, named flood-search policy. The algorithm is inspired by the situation that nodes and edges in CFG are an analogy for reservoirs and gates between reservoirs, with the starting point of the CFG as the flood point.

Algorithm.\ref{algo:search} is the description of the search algorithm.
Suppose the starting node \emph{n} is flooded, all the sides of the graph are reservoirs, all the nodes of the graph are gates, each gate have two states (open/closed). If there are one or more empty reservoirs (edge) in the current path, the path is considered a valuable path, we will save the current execution state and find the shortest path to the program exit as soon as possible to get the value of this path, which means that the new constraints will be collected. If all reachable 
paths of the current nodes or edges have no value (path have no unvisited edges), these nodes or edges have no value as well.

In our CFG model, each node in the graph represents a basic statement block, directed edges are used to represent jumps in the control flow. The branch edges of branch node record the branch condition and their result (true/false). Because the main goal of the search is to cover all branch edges in the graph, when encountering a branch node, flood-search policy forks a copy of current execution state, and adds the new execution state to open or close list, depending on the visit status of its branch.

If the input is G(edges, nodes), which is a CFG model. At the beginning, we push the state initialized by the start node into the open list, while the closed list is empty. Then the search starts to get execution states from the open list, and executes them by order, suppose the current execution state is \emph{s}. Every execution state in the open list is considered to be valuable, which means it may have new constraints, so flood-search will search the shortest way from the current executed node in \emph{s} to the exit node to keep this path, and make sure constraints in this path will be collected.

After the current execution state is executed, the next execution state of \emph{s} will be executed. If the current executed node in \emph{s} is a branch node and the node has more than one unvisited node, \emph{s} should be added to open list, because the unvisited branch of \emph{s} must be traversed. Even if \emph{s} has no unvisited branch, it still possibly has a succeed path unvisited, so \emph{s} should be stored in the close list, and prepared for further searching.

Compared with other graph searching algorithms such as BFS or DFS, flood-search fits well for CFG traverse, for flood-search trying to visit unvisited edges and nodes as early as possible, meanwhile, BFS or DFS may be caught in the loop.

\begin{algorithm2e}
\small
  \setcounter{AlgoLine}{0}
\caption{Flood-search for Control Flow Graph}\label{algo:search}
\DontPrintSemicolon
\newcommand\mycommfont[1]{\small\sffamily\textcolor{gray}{#1}}
\SetCommentSty{mycommfont}
% \KwInput{ \begin{tabularx}{.9\linewidth}{>{$}c<{$} X}
%     c_1,\ldots c_N  & the cut path
%   \end{tabularx}}

\KwIn{$G(edges,nodes)$: a control flow graph}

\BlankLine

$open$ $\gets$ \{State(Root($G$))\}, $close$ $\gets$ \{\}

\Repeat{$open$.size $=$ 0}
{
 SearchShortestToExit(Pop($open$));
 \;
 \If{$open$.size $=$ 0} {
  Discharge();
 }
}

\BlankLine

\textbf{Procedure} SearchShortestToExit(State $s$)

 \If{$s$ is on the end node of the graph}{
 \Return
 }
 $next\_state$ $\gets$ Next($s$);
 \;
 \If{$s$ has unvisited edge}{
 $open \gets open \cup \{s\}$\;
 }
 \ElseIf{$s$ has visited edge}{
 $close \gets close \cup \{s\}$\;
 }
 \Else{
 $close \gets close \cup \{s\}$\;
 \Return}
 SearchShortestToExit($next\_state$);
 \;
 \;
 
\textbf{Procedure} Discharge()
 \;
 \Repeat{$close$.size $=$ 0}
 {
  $open$ $\gets$ $open$ $\cup$ \{Next(Pop($close$))\}\;
 }

\end{algorithm2e}

\subsubsection{Memory model}
The memory model is the key module to track execution states and gather constraints, by simulating whole memory allocation.
Very basically, memory model stores all variables of basic types, such as int, char, including their names and values.
Dealing with complex types, such as the pointer, is a challenge for analysis tools. 
Our solution is below. For the array of basic types, in addition to memory space needed by the variable in the array, the total size of the array will also be stored, to perform plus/minus on pointers, and check if the pointer is out of memory bound. Furthermore, to deal with the member of the struct, union or enum, the total data structure and the start location in memory are needed to locate the variable by start location and the memory offset. 

\subsection{Cloud-based Testing Environment}
The SmartUnit Service contains all other features except the core analysis module, including web frontend UI, backend master process to handle web requests, worker process to perform analysis actions, database module to store test results.
The SmartUnit System architecture diagram is shown in Figure.~\ref{fig:web}.
\begin{figure}
    \includegraphics[width=0.3\textwidth]{Figs/web.pdf}
    \caption{The workflow of the cloud-based platform.}
    \label{fig:web}
\end{figure}
Web UI is designed to manage projects to be tested and get the results. Tested project is needed to be uploaded to the server after archived, and will be passed to master process for further operations.
The master process extracts the uploaded archive, creates a record in the database, and forks a worker process to call SmartUnit analysis engine to generate test cases for the project.

After SmartUnit finishes its analysis, worker process updates the status and saves generated in the database, then status in Web UI is also updated, after which users could download test cases in specific formats.
When the master process receives a request about specific test case, it will check if the test case is already prepared. If not, master process will generate a test case file according to test case data in the database and required file format. After finished, the test case archive is returned to the Web UI and could be reused in further downloading.

\subsection{Challenges and Solutions}
\subsubsection{Pointer}
The symbolizing  of the pointer variable is a big challenge, because the pointer operations need to access the real value of the pointer and the variable that pointer points to. The real value of the pointer is hard to access as it is regarded as a symbolic value that means we must maintain a pointer array of pointer owner to execute a pointer operation, and the length of this array may be infinite because the pointer execution could be everything. 

SmartUnit can support pointer operations, while a pointer memory must include the array memory of its owner which the pointer belongs to, the offset to address the position of the pointer, and some other marks such as null pointer mark. For the array of basic types, in addition to memory space needed by the variable in the array, the size of array will also be stored, to perform plus/minus operations on pointers, and check if pointer is out of memory bound.

\subsubsection{void*}
In most embedded C programs, (void*) is a special data type treated as a type that means nothing and used to transform data without data type. In Memory model, each pointer typed (void*) will be stored with its original type.
SmartUnit implements this by maintaining a void memory type and saves the alias of the memory in it. When executor comes to the (void*), it will create a voidmemory type, and record its type information to the aliased memory of the voidmemory. It will update the aliased memory when executing to the assignment of void*, and look up to its alias memory rather than voidmemory itself, so that we can get the type and memory information of the void* type.

\subsubsection{Complex data structure}
Complex data structures like struct, union or enum type are hard to handle, for they do not have a fixed length. To deal with the members of the struct, union or enum type, the total data structure and the start location in memory are needed to locate the variable by start location and the memory offset.

For a struct memory, the difficulty is to do operations related to the index. Thus, in addition to storing all variable declaration, the start and end memory location and relation between previous and next memory block are also needed to be stored.

==> KLEE workshop/introduction.tex <==
\section{Introduction}

Data-flow testing is a group of testing strategies which aims to find paths to exercise the interactions between definitions and uses of the variables.
The faults can be found by observing whether all corresponding uses produce the desired results.
The idea of data-flow testing was first proposed in 1976 by Herman~\cite{herman1976data} who claimed data-flow testing could test a program more thoroughly and reveal more subtle software bugs.
Several empirical studies have revealed that data-flow coverage criteria is more effective than control-flow coverage criteria~\cite{hutchins1994experiments, frankl1998further}.
However, data-flow coverage still cannot find its adoption in practice, due to the lack of effective tool support.

In this presentation, we propose an efficient guided testing approach which achieves data-flow coverage criteria.
To our knowledge, we are the first to adapt symbolic execution engine KLEE for data-flow testing and have implemented it on KLEE, an efficient and robust symbolic execution engine. 
To evaluate its efficiency, we build a data-flow testing benchmark, 
which consists of the subjects used in previous data-flow testing work, Software-artifact Infrastructure Repository\footnote{http://sir.unl.edu/portal/index.php} (SIR), and International Competition on Software Verification (SV-COMP) benchmark. 
% We will integrate this approach into our unit testing engine SmartUnit and help several corporations and institutions to adopt data-flow testing in practice.


==> KLEE workshop/related_work.tex <==
\section{Application}

The idea in this presentation comes from our previous work published in ICSE'15~\cite{su2015combining}. According to our survey on data-flow testing~\cite{su2017survey}, there are a variety of approaches to generate data-flow test data, such as \emph{random testing}, \emph{collateral coverage-based testing}, \emph{search-based testing} and
\emph{model checking-based testing}. However, to our knowledge, we are the first to adapt symbolic execution for data-flow testing. Symbolic execution is a more efficient and precise way, because it can straightforwardly find the paths that satisfy the data-flow coverage criteria and easily generate the test case.

Furthermore, we implemented a cloud-based industrial automated unit test generation framework named SmartUnit~\cite{zhang2018smartunit} which
 depends on our previous work on symbolic execution~\cite{su2014automated,su2016automated}.
It helps several corporations and institutions to adopt coverage-based testing in practice, include \emph{China Academy of Space Technology}, the main spacecraft development and production agency in China (like NASA in the United States);
\emph{CASCO Signal Ltd.}, the best railway signal technique corporation in China, \etc.
SmartUnit has totally tested more than one million lines of code since its release in 2016.

==> KLEE workshop/results_and_analysis.tex <==
\section{results and analysis}
\textbf{RQ1: How about the performance of automated unit test generation framework SmartUnit in both commercial embedded software and open-source database software?}
For this question, we pushed the benchmarks to the SmartUnit testing platform, made it run automatically, and got the coverage from the web view.
Table~\ref{table:RQ1_coverage} shows the coverage information of the benchmarks. In Column \emph{Subject}, the items represent the name of the programs in our benchmark. The Column \emph{\#Test cases} represents the number of test cases 
generated by SmartUnit for the corresponding benchmark.
SmartUnit calculated coverage for each module individual because we separated PostgreSQL into the divided modules. Thus, we used PostgreSQL plus module names as the benchmark names in Table~\ref{table:RQ1_coverage}. 
The numbers in Statement Coverage, Branch Coverage, and MC/DC Coverage represent the number of functions in the corresponding range. The number of functions which achieve 100\% coverage is high lighted in gray.

In general, more than 90\% of functions in commercial embedded software achieve 100\% statement, branch, MC/DC coverage, 
more than 80\% of functions in SQLite achieve 100\% statement, branch, MC/DC coverage, and more than 60\% of functions in PostgreSQL achieve 100\% statement, branch, MC/DC coverage. 
As Table~\ref{table:RQ1_coverage} shows, most of the functions achieve 100\% statement, branch, MC/DC coverage.
Except for 100\% coverage, the number of functions is the even distribution in other coverage ranges. 

From the data, the conclusion is SmartUnit have a good performance on commercial embedded software and SQLite which is used in embedded systems.
The performance on PostgreSQL not as good as commercial embedded software and SQLite, but is also well enough.
It means SmartUnit is more suitable for embedded software and also have a well enough performance on common software.
However, there are also some functions not achieving 100\% of statement, branch, MC/DC coverage, 
what factors make SmartUnit not get 100\% coverage will be discussed in RQ2.

\begin{table*}
    \Huge
    \centering
    \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
    \resizebox{\textwidth}{!}{\begin{minipage}{\textwidth}
    \centering
    \caption{Performance of \textit{SmartUnit} on coverage.}
    \label{table:RQ1_coverage}
    \resizebox{\textwidth}{!}{% Resize table to fit within \linewidth horizontally
    \begin{tabular}{|c|c|ccccc|ccccc|ccccc|}
    \toprule
    \multicolumn{1}{|c|}{Subject} 
    &\multicolumn{1}{c|}{\#Test cases} 
    &\multicolumn{5}{c|}{Statement Coverage (\#Functions)} 
    &\multicolumn{5}{c|}{Branch Coverage (\#Functions)} 
    &\multicolumn{5}{c|}{MC/DC Coverage (\#Functions)} 
    \\

    &
    &0\%-10\% &10\%-50\% &50\%-90\% &90\%-100\% &100\% 
    &0\%-10\% &10\%-50\% &50\%-90\% &90\%-100\% &100\% 
    &0\%-10\% &10\%-50\% &50\%-90\% &90\%-100\% &100\% 

    \\ \hline
    \tabincell{c}{\emph{aerospace software}}
    & \tabincell{c}{712}
    %SC
    & \tabincell{c}{1}
    & \tabincell{c}{4}
    & \tabincell{c}{5}
    & \tabincell{c}{4}
    & \tabincell{c}{\cellcolor{gray!30}40}
    %BC
    & \tabincell{c}{1}
    & \tabincell{c}{4}
    & \tabincell{c}{5}
    & \tabincell{c}{3}
    & \tabincell{c}{\cellcolor{gray!30}40}
    %MC/DC
    & \tabincell{c}{3}
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}51}
    
    
    \\ \hline
    \tabincell{c}{\emph{automotive software}}
    & \tabincell{c}{3134}
    %SC
    & \tabincell{c}{1}
    & \tabincell{c}{3}
    & \tabincell{c}{9}
    & \tabincell{c}{2}
    & \tabincell{c}{\cellcolor{gray!30}315}
    %BC
    & \tabincell{c}{1}
    & \tabincell{c}{6}
    & \tabincell{c}{8}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}315}
    %MC/DC
    & \tabincell{c}{3}
    & \tabincell{c}{3}
    & \tabincell{c}{1}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}323}
    
    
    \\ \hline
    \tabincell{c}{\emph{subway signal software}}
    & \tabincell{c}{14848}
    %SC
    & \tabincell{c}{1}
    & \tabincell{c}{5}
    & \tabincell{c}{23}
    & \tabincell{c}{37}
    & \tabincell{c}{\cellcolor{gray!30}808}
    %BC
    & \tabincell{c}{1}
    & \tabincell{c}{5}
    & \tabincell{c}{35}
    & \tabincell{c}{33}
    & \tabincell{c}{\cellcolor{gray!30}800}
    %MC/DC
    & \tabincell{c}{7}
    & \tabincell{c}{5}
    & \tabincell{c}{9}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}853}
    
    
    \\ \hline
    \tabincell{c}{\emph{SQLite}}
    & \tabincell{c}{6814}
    %SC
    & \tabincell{c}{95}
    & \tabincell{c}{85}
    & \tabincell{c}{147}
    & \tabincell{c}{62}
    & \tabincell{c}{\cellcolor{gray!30}1657}
    %BC
    & \tabincell{c}{98}
    & \tabincell{c}{111}
    & \tabincell{c}{144}
    & \tabincell{c}{66}
    & \tabincell{c}{\cellcolor{gray!30}1627}
    %MC/DC
    & \tabincell{c}{146}
    & \tabincell{c}{68}
    & \tabincell{c}{140}
    & \tabincell{c}{8}
    & \tabincell{c}{\cellcolor{gray!30}1684}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL bootstrap}}
    & \tabincell{c}{27}
    %SC
    & \tabincell{c}{1}
    & \tabincell{c}{9}
    & \tabincell{c}{2}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}9}
    %BC
    & \tabincell{c}{1}
    & \tabincell{c}{11}
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}9}
    %MC/DC
    & \tabincell{c}{12}
    & \tabincell{c}{-}
    & \tabincell{c}{1}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}8}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL catalog}}
    & \tabincell{c}{1197}
    %SC
    & \tabincell{c}{10}
    & \tabincell{c}{91}
    & \tabincell{c}{131}
    & \tabincell{c}{7}
    & \tabincell{c}{\cellcolor{gray!30}186}
    %BC
    & \tabincell{c}{14}
    & \tabincell{c}{148}
    & \tabincell{c}{75}
    & \tabincell{c}{13}
    & \tabincell{c}{\cellcolor{gray!30}175}
    %MC/DC
    & \tabincell{c}{183}
    & \tabincell{c}{31}
    & \tabincell{c}{8}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}203}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL initdb}}
    & \tabincell{c}{312}
    %SC
    & \tabincell{c}{-}
    & \tabincell{c}{2}
    & \tabincell{c}{3}
    & \tabincell{c}{6}
    & \tabincell{c}{\cellcolor{gray!30}61}
    %BC
    & \tabincell{c}{-}
    & \tabincell{c}{4}
    & \tabincell{c}{10}
    & \tabincell{c}{11}
    & \tabincell{c}{\cellcolor{gray!30}49}
    %MC/DC
    & \tabincell{c}{2}
    & \tabincell{c}{-}
    & \tabincell{c}{9}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}61}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL pg\_dump}}
    & \tabincell{c}{1608}
    %SC
    & \tabincell{c}{16}
    & \tabincell{c}{27}
    & \tabincell{c}{60}
    & \tabincell{c}{25}
    & \tabincell{c}{\cellcolor{gray!30}378}
    %BC
    & \tabincell{c}{20}
    & \tabincell{c}{36}
    & \tabincell{c}{60}
    & \tabincell{c}{38}
    & \tabincell{c}{\cellcolor{gray!30}352}
    %MC/DC
    & \tabincell{c}{37}
    & \tabincell{c}{22}
    & \tabincell{c}{32}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}415}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL pg\_resetxlog}}
    & \tabincell{c}{65}
    %SC
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{2}
    & \tabincell{c}{1}
    & \tabincell{c}{\cellcolor{gray!30}8}
    %BC
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{2}
    & \tabincell{c}{1}
    & \tabincell{c}{\cellcolor{gray!30}8}
    %MC/DC
    & \tabincell{c}{-}
    & \tabincell{c}{1}
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}10}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL pg\_rewind}}
    & \tabincell{c}{245}
    %SC
    & \tabincell{c}{4}
    & \tabincell{c}{1}
    & \tabincell{c}{2}
    & \tabincell{c}{4}
    & \tabincell{c}{\cellcolor{gray!30}53}
    %BC
    & \tabincell{c}{4}
    & \tabincell{c}{1}
    & \tabincell{c}{2}
    & \tabincell{c}{5}
    & \tabincell{c}{\cellcolor{gray!30}52}
    %MC/DC
    & \tabincell{c}{4}
    & \tabincell{c}{-}
    & \tabincell{c}{4}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}56}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL pg\_upgrade}}
    & \tabincell{c}{305}
    %SC
    & \tabincell{c}{6}
    & \tabincell{c}{3}
    & \tabincell{c}{5}
    & \tabincell{c}{5}
    & \tabincell{c}{\cellcolor{gray!30}81}
    %BC
    & \tabincell{c}{6}
    & \tabincell{c}{4}
    & \tabincell{c}{4}
    & \tabincell{c}{9}
    & \tabincell{c}{\cellcolor{gray!30}77}
    %MC/DC
    & \tabincell{c}{8}
    & \tabincell{c}{2}
    & \tabincell{c}{9}
    & \tabincell{c}{1}
    & \tabincell{c}{\cellcolor{gray!30}80}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL pg\_xlogdump}}
    & \tabincell{c}{67}
    %SC
    & \tabincell{c}{3}
    & \tabincell{c}{2}
    & \tabincell{c}{2}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}11}
    %BC
    & \tabincell{c}{3}
    & \tabincell{c}{2}
    & \tabincell{c}{3}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}10}
    %MC/DC
    & \tabincell{c}{3}
    & \tabincell{c}{1}
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}14}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL pgtz}}
    & \tabincell{c}{9112}
    %SC
    & \tabincell{c}{587}
    & \tabincell{c}{595}
    & \tabincell{c}{704}
    & \tabincell{c}{68}
    & \tabincell{c}{\cellcolor{gray!30}2465}
    %BC
    & \tabincell{c}{617}
    & \tabincell{c}{872}
    & \tabincell{c}{475}
    & \tabincell{c}{51}
    & \tabincell{c}{\cellcolor{gray!30}2404}
    %MC/DC
    & \tabincell{c}{1393}
    & \tabincell{c}{233}
    & \tabincell{c}{139}
    & \tabincell{c}{8}
    & \tabincell{c}{\cellcolor{gray!30}2646}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL psql}}
    & \tabincell{c}{1378}
    %SC
    & \tabincell{c}{3}
    & \tabincell{c}{13}
    & \tabincell{c}{18}
    & \tabincell{c}{14}
    & \tabincell{c}{\cellcolor{gray!30}380}
    %BC
    & \tabincell{c}{3}
    & \tabincell{c}{15}
    & \tabincell{c}{19}
    & \tabincell{c}{18}
    & \tabincell{c}{\cellcolor{gray!30}373}
    %MC/DC
    & \tabincell{c}{10}
    & \tabincell{c}{12}
    & \tabincell{c}{27}
    & \tabincell{c}{2}
    & \tabincell{c}{\cellcolor{gray!30}377}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL scripts1}}
    & \tabincell{c}{189}
    %SC
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{7}
    & \tabincell{c}{4}
    & \tabincell{c}{\cellcolor{gray!30}30}
    %BC
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{7}
    & \tabincell{c}{6}
    & \tabincell{c}{\cellcolor{gray!30}28}
    %MC/DC
    & \tabincell{c}{-}
    & \tabincell{c}{2}
    & \tabincell{c}{6}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}33}
    \\
    
\bottomrule
\end{tabular}}
\end{minipage}}
\end{table*}

\lstset{
    frame=tb,
    language=C,
    aboveskip=3mm,
    belowskip=3mm,
    showstringspaces=false,
    columns=flexible,
    basicstyle={\small\ttfamily},
    breaklines=true,
    breakatwhitespace=true,
    tabsize=3,
    basicstyle=\footnotesize\ttfamily
}

\textbf{RQ2: What factors make dynamic symbolic execution get low coverage?}
In Table.~\ref{table:RQ1_coverage}, although SmartUnit has the high statement, branch, and MC/DC coverage,
there are some function units has a low coverage (\eg 0\%-10\%).
We found the low coverage functions, read the source code and analysis manually to find out why SmartUnit
get the low coverage in these functions. We categorized the main reasons as follows:

\textbf{Environment variable and Environment function:} 
In the benchmarks, there is a variety of environment variable and environment function in the code. 
For example, the current time is an environment variable, it comes from the system and is difficult to be symbolized.
Environment function are usually standard library calls, such as \textit{sizeof()}. 
Listing.~\ref{lst:sizeof} is an example from PostgreSQL. 
It is difficult to covert the condition in line 4 to a constraint, because symbolic execution engine is hard to comprehend the semantic of the environment functions. Therefore, the coverage can not achieve 100\% in this situation.
\begin{lstlisting}[caption={An example of environment function.},label={lst:sizeof},language=C]
static void handle_sigint(SIGNAL_ARGS)
{
        ...
        if (PQcancel(cancelConn, errbuf, sizeof(errbuf)))
        {
            CancelRequested = true;
            fprintf(stderr, _("Cancel request sent\n"));
        }
        else
            fprintf(stderr, _("Could not send cancel request: %s"), errbuf);
        ...
}
\end{lstlisting}


\textbf{Complex operation:} Although we have a solution to deal with the variable pointer, the complex operation is difficult to deal with.
Listing.~\ref{lst:complex} comes from SQLite. There is a complex pointer operation in line 4 which combines variable pointers and function pointers. 
Due to the limit of the memory model, it can not handle these complex operations.
Execution will be terminated by this kind of statement and get a low coverage.
\begin{lstlisting}[caption={An example of environment function.},label={lst:complex},language=C]
static void callFinaliser(sqlite3 *db, int offset){
 ...
 int (*x)(sqlite3_vtab *);
 x = *(int (**)(sqlite3_vtab *))((char *)p->pModule + offset);
 if( x ) x(p);
 ...
}
\end{lstlisting}

\textbf{limitation of SMT solver:} In SmartUnit, Z3 Solver is the main SMT solver to solve the constraint. 
Although Z3 is one of the best SMT solvers, it still has some limitation. Here is an example.
\textit{y != 0 \&\& (((x-1) * y) \% y) == 1} is a constraint collected by SmartUnit in the commercial software. 
Although it is a legal constraint and there is no divided by zero faults, the Z3 solver can not deal with it.
The Z3 solver developer said that Z3 could not deal with nonlinear constraints, such as this constraint.
It is the common reason for getting the low coverage.
Thus the coverage of symbolic execution is sometimes affected by the SMT solver.

\textbf{RQ3: Can SmartUnit find the potential runtime exception in real-world software?}
From RQ1, we found that SmartUnit has a high coverage on the real world software. 
During the execution, there are also some of the potential runtime exceptions in this software.
Except the factors discussed in RQ2, we found more than 5,000 number of test cases with runtime exceptions. Due to the time limit, we have not checked every test case manually, we sampled from the test cases to analysis the runtime exceptions. Generally, we divided the runtime exceptions found by SmartUnit into three categories: 
array index out of bounds, fixed memory address and divided by zero. 

\textbf{Array index out of bounds:} As the introduction in Section 3, SmartUnit use memory model to simulate whole memory allocation.
if there is an array index out of bounds, SmartUnit will throw a runtime exception. 
Listing.~\ref{lst:array} is an example comes from SQLite. 
Obviously, in this function, there is an out of bounds runtime exception in line 10, when \emph{i \textless argc}. 
Although the caller of this function ensure \emph{i \textless= argc} in SQLite, 
it has a potential runtime exceptions if other callers not ensure \emph{i \textless= argc}.
There is even no precondition in the comment.
It is quite serious if a programmer wants to call it, but doesn't know the precondition.
We have found much of runtime exceptions in this category from all of the benchmarks.

\begin{lstlisting}[caption={An example of array index out of bounds.},label={lst:array},language=C]
/*
** Get the argument to an --option.  Throw an error and die if 
** no argument is available.
*/
static char *cmdline_option_value(int argc, char **argv, int i) {
    if (i == argc) {
        utf8_printf(stderr, "%s: Error: missing argument to %s\n", argv[0], argv[argc - 1]);
        exit(1);
    }
    return argv[i];
}
\end{lstlisting}

\textbf{Fixed memory address:} Fixed memory address is a problem in dealing with the variable pointer. 
In the embedded system, there are many pointer operations with the fixed memory address. 
It is hard for memory model to simulate a fixed memory address.
For example, the operations like (*0X00000052) or (* (symbolic variable + 12)) will cause runtime exceptions.
It usually gets \textit{NULL} when referring from a fixed memory address.
Thus symbolic execution will throw runtime exception with fixed memory address operations.


\textbf{Divided by zero:} Divided by zero is also a common runtime exception in the benchmarks. 
It usually appears in numerical calculation of program. 
SmartUnit will generate boundary value to check if the program exists divided by zero runtime exception.
We select a brief example from SQLite to discuss this runtime exception. 
Listing.~\ref{lst:zero} is the function which has the potential runtime exception in line 19.
When \emph{nUsable == 4}, the expression \emph{(nTotal - nMinLocal) \% (nUsable - 4)} will throw a divided by zero runtime exception.
we read the source code manually and found that it is difficult to comfirm whether \emph{nUsable} could be 4 or not.
The comment of the function does not contain the precondition of \emph{nUsable}.
It's horrible if the programmer who calls this function in a new function and do not know the implicit prediction.

\begin{lstlisting}[caption={An example of divided by zero.},label={lst:zero},language=C]
static void getLocalPayload(
  int nUsable,                    /* Usable bytes per page */
  u8 flags,                       /* Page flags */
  int nTotal,                     /* Total record (payload) size */
  int *pnLocal                    /* OUT: Bytes stored locally */
){
  int nLocal;
  int nMinLocal;
  int nMaxLocal;
 
  if( flags==0x0D ){              /* Table leaf node */
    nMinLocal = (nUsable - 12) * 32 / 255 - 23;
    nMaxLocal = nUsable - 35;
  }else{                          /* Index interior and leaf nodes */
    nMinLocal = (nUsable - 12) * 32 / 255 - 23;
    nMaxLocal = (nUsable - 12) * 64 / 255 - 23;
  }

  nLocal = nMinLocal + (nTotal - nMinLocal) % (nUsable - 4);
  if( nLocal>nMaxLocal ) nLocal = nMinLocal;
  *pnLocal = nLocal;
}
\end{lstlisting}

In summary, SmartUnit could find the potential runtime exceptions in real-world software. We categorized and analyzed the potential runtime exceptions. 
Most of these potential runtime exceptions existed, due to there is no protection for input values.
At the same time, there is no clear precondition specification for the functions.
Although there are protection codes in the caller of the function, the potential runtime exceptions may cause the real faults in real-world software.



\textbf{RQ4: What is the difference between automatically generated test cases and manually written test cases?}
In RQ4, we compare automatically generated test cases and manually written test cases in the following aspect: time, cost and quality.

\textbf{Time \& Cost:} Table~\ref{table:RQ4_time} shows the test set generated time for each benchmark. 
The column \textit{Subject} list all of the benchmark we used.
As Table~\ref{table:RQ1_coverage}, we separate PostgreSQL into the individual module, and name with PostgreSQL plus module name.
The second column \textit{\# Functions} represents the number of functions in the benchmark.
The column \textit{Time} means the test set generated time for the corresponding benchmark.
The column \textit{Average} represents the average test set generated time for the corresponding benchmark per function, 
in other words, it means the average time of SmartUnit generates test set for a function.
Deserve to be mentioned, we use \textit{Total\# Function} and \textit{Total Time} to calculate \textit{Total Average}.

In Table~\ref{table:RQ4_time}, it is obvious that the average time ranges from 1s to 7s and total average time is 3.77s for all of the benchmarks.
It means that SmartUnit spends nearly 4s to generate test cases for a function, 
and in the best situation, more than 90\% of the functions can achieve 100\% statement, branch, and MC/DC coverage.
How about the test engineer? In our survey from companies, a trained test engineer can product test case for 5-8 functions per day. 
Thus using automated unit test generation framework can cost less time than employing test engineers. 

The main cost of automatically generated test cases and manually written test cases are both the salary paid for the employee. We assume a
developer costs twice salary higher than a test engineer. SmartUnit has cost 24 man-month to release. For manually testing, 
a test engineer could write the test case for about 160 functions per month. Thus 24 man-month cost could support test engineers write about 8,000 functions. 
In summary, if you have a large number of function units(\eg more than 10,000), automatically generated test cases are cheaper.
On the contrary, manual test cases are cheaper for the little scale of projects. 

\textbf{Quality:} From RQ1, we have the conclusion that more than 90\% of functions in commercial embedded software can achieve 100\% statement, branch and MC/DC coverage; more than 80\% of functions in SQLite achieve 100\% coverage, and more than 60\% of functions in PostgreSQL achieve 100\% coverage. According to our survey in the companies, the test engineers need to achieve 100\% coverage for each function. If we use coverage as a quality indicator, automatically generated test case has overwhelming superiority on cost and time though manual test case has higher coverage in some cases. Meanwhile, the automatically generated test cases could find runtime exception in time. 

\begin{table}[!t]
\footnotesize
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
\caption{Test set generated time for each benckmark.}
\label{table:RQ4_time}
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
\begin{tabular}{|c||c|c|c|}
\hline
Subject &\# Functions &Time (s) &Average (s/func) \\
\hline
\hline
aerospace software &54 &318 &6\\
automotive software &330 &329 &1\\
subway signal software &874 &2,476 &3\\
SQLite &2046 &13,482 &6\\
PostgreSQL bootstrap &21 &48 &2\\
PostgreSQL catalog &425 &1,350 &3\\
PostgreSQL initdb &72 &548 &7\\
PostgreSQL pg\_dump &506 &3,428 &7\\
PostgreSQL pg\_resetxlog &11 &71 &6\\
PostgreSQL pg\_rewind &64 &352 &5\\
PostgreSQL pg\_upgrade &100 &465 &5\\
PostgreSQL pg\_xlogdump &18 &130 &7\\
PostgreSQL pgtz &4419 &10,478 &2\\
PostgreSQL psql &428 &1,676 &4\\
PostgreSQL scripts1 &41 &311 &7\\


\hline
\hline
Total &9,409 &35,462 &3.77\\
\hline
\end{tabular}
\end{table}

\textbf{Discussion}

Traditional automated unit testing tools focus on the automated random testing, \eg, test cases are randomly derived as the input to invoke the program code under test. Although the random test data generation algorithm is quite easy to be implemented, it is obviously that the expected coverage criteria (e.g., the branch and the statement coverage) cannot be guaranteed. The DART (Directed Automated Random Testing) is a classical unit testing tool that supports the directed random test data generation~\cite{godefroid2005dart}. One unique characteristic of the DART is its complete automation for unit testing. Since its underlying approach is random testing, the DART focuses on detecting standard errors such as program crashes, assertion violations, and non-termination while it is not deliberately designed for certain coverage criteria requested by the industrial standards. Our SmartUnit framework can handle the automated testing and support various coverage criteria of the industrial standards.

   PEX is a famous unit testing tool that automatically generates test suites with high code coverage~\cite{tillmann2008pex}. It is a Visual Studio add-in for testing .NET Framework applications. In practice, the PEX tool is adapted to testing the C\# code. Similarly the IntelliTest\footnote{https://msdn.microsoft.com/en-us/library/dn823749.aspx} also automatically generates test data for the unit test of C\#. The basic idea of the IntelliTest is to generate test data to execute each statement of the target code and then analyze the coverage of the conditional branch. The Microsoft Security Risk Detection is a unique fuzz testing service for finding security critical bugs in software. These three tools significantly improve the unit testing in bug detection and time efficiency. However, since these tools are designed as general solutions for unit testing, it cannot be directly applied in the domain of real-time control software testing. They fall short in supporting the unit testing of the control software since some unique features such as the high coverage request of particular criteria requested by the industrial standards have not been deliberately considered. The SmartUnit framework focuses on the request of current industry standards and offers a completely automated solution for the unit testing of the real-time software.
   
Although there is a plug-in of Testbed called LDRA TBrun\footnote{http://ldra.com/industrial-energy/products/tbrun/} which can automatically generate driver program and test harness without manual script,
SmartUnit is quite different from it.
LDRA TBrun uses data dictionary to generate the test cases, it combines several values in the data dictionary, 
usually considering up bound and low bound of variables. 
This strategy is not able to deal with memory calculation, while SmartUnit can easily catch memory change constraints by DSE.
LDRA TBrun generates unit test suite based-on boundary value (\eg, maximum value, minimum value, median value, \etc),
while SmartUnit is a coverage-driven tool, it can satisfy statement, branch, MC/DC coverage criteria from industrial requirements.
SmartUnit can avoid repetitive test cases, while LDRA TBrun has many repetitive test cases in its test set.
LDRA TBrun can not give the expectative output value for each test case, 
but SmartUnit can expect output value by executing test cases automatically after generation.
SmartUnit can not only generate the test cases for function parameters and global variables which support in LDRA TBrun,
it can also generate the test cases for instrument function parameters and instrument function return value. 
In summary, LDRA TBrun is suitable for critical testing and robustness testing,
while SmartUnit is suitable for coverage-driven testing.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-sigconf.tex \



PDF = ${SAMPLES:%.tex=%.pdf}

all:  ${PDF} clean


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-sigconf.pdf : introduction.tex \
					 approach_and_implementation.tex \
					 evaluation_and_discussion.tex \
					 related_work.tex \
					 conclusion.tex 



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	# $(RM) $(PACKAGE).cls *.log *.aux \
	# *.cfg *.glo *.idx *.toc \
	# *.ilg *.ind *.out *.lof \
	# *.lot *.bbl *.blg *.gls *.cut *.hd \
	# *.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf


==> evaluation_setup.tex <==
\section{Evaluation Setup}
\subsection{Research Questions}
To achieve the goal, we intend to set up some research questions which can guide our evaluation. 
The research questions are described as follows:
\begin{itemize}
  \item \textbf{\textit{RQ1}}: How about the performance of automated unit test generation framework SmartUnit in both commercial embedded software and open-source database software?
        In this paper, we use statement coverage, branch coverage, and MC/DC as evaluation indicators.
  \item \textbf{\textit{RQ2}}: What factors make dynamic symbolic execution get low coverage? 
  \item \textbf{\textit{RQ3}}: Can SmartUnit find the potential runtime exceptions in real-world software?
  \item \textbf{\textit{RQ4}}: What is the difference in terms of time, cost and quality between automatically generated test cases and manually written test cases? 
\end{itemize}

We package the the code under test and submit them to the SmartUnit cloud platform. SmartUnit can start dynamic symbolic execution automatically.
After the execution, a series of packaged .tcf files (the test cases) for the codes can be downloaded from the platform. 
We import the test cases into Testbed to get the coverage and detect the runtime error.
Testbed will generate a detailed testing report after running the automatically generated unit test cases.
Statement, branch and MC/DC coverage, runtime errors, and static errors are provided by the report.

The statement, branch and MC/DC coverage of each function will be recorded as the performance indicator for \textit{RQ1}. 
We turn our attention to the functions which gets low coverage in the three coverage criteria above, to answer \textit{RQ2}.
The runtime errors will be classified into a several of categories, so that we can obtain some insights from them, in \textit{RQ3}.
It's impossible to manually write test cases for all of the benchmark, because of the large scale of the software in the benchmark. 
We will select some representative codes to answer \textit{RQ4}.

\subsection{Benchmark}
This paper selects two kinds of C program benchmarks for SmartUnit: commercial embedded software and open-source database software.
Table ~\ref{table:benchmark} gives the list of benchmarks for the evaluation. Due to the confidentiality agreement, 
we hide the commercial software names in this paper.

\begin{table}[!t]
\footnotesize
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
\caption{Subjects of Evaluation Benchmark Repository.}
\label{table:benchmark}
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
\begin{tabular}{|c||c|c|c|}
\hline
Subject &\# Files &\# Functions &\# LOC\\
\hline
\hline
aerospace software &8 &54 &3,769\\
automotive software &4 &330 &31,760\\
subway signal software &108 &874 &37,506\\
SQLite &2 &2046 &126,691\\
PostgreSQL &906 &6105 &279,809\\
\hline
\hline
Total &1028 &9,409 &479,535\\
\hline
\end{tabular}
\end{table}

\textbf{The commercial embedded software} comes from aerospace, automotive, subway signal companies.
SmartUnit has tested millions of code from commercial embedded software. For example, 
in the aerospace company, SmartUnit tested more than 100,000 LOC. Over 70\% functions have achieved
more than 90\% statement coverage. In order to intensively study, we selected three benchmarks from the different areas to get a variety of characteristics. All of them come from real-world industrial code.

\textbf{The open-source database software} used in this paper are \textit{SQLite}\footnote{https://www.sqlite.org/} and \textit{PostgreSQL}\footnote{https://www.postgresql.org/}. 
Due to security demand of the commercial embedded software, we mainly use the open-source database software to explain.
We chose SQLite because it is an embedded SQL database engine, usually used in embedded software systems. 
It is a good sample for us to find some insights when using SmartUnit on the embedded system, which has nearly 200,000 LOC. 
The PostgreSQL is a representative object-relation database system, usually used as the enterprise-class database.
We chose PostgreSQL as a benchmark in order to evaluate performance and expandability of SmartUnit on the enterprise-class system.

For each subject, we put all of the .c and .h files into one folder to make it easier for Smartunit to get the relied header files for under test functions.
We divided each subject into an independent .zip package so that we can calculate coverage respectively.


\subsection{Evaluation Environment}
SmartUnit was run on a virtual machine with three processors and 3GB memory, CentOS operating system.

Testbed was run on a virtual machine with two processors(2.70GHz Intel(R) Core(TM) i5-2500S CPU) and 1GB memory, 
32bit Microsoft Windows XP Professional Service Pack 3 operating system.






==> framework_implementation.tex <==
\section{Framework Implementation}
\subsection{Framework Architecture}
Figure.~\ref{fig:backend} shows the core framework of SmartUnit.
\begin{figure}
    \includegraphics[width=0.3\textwidth]{Figs/backend.pdf}
    \caption{The architecture of SmartUnit.}
    \label{fig:backend}
\end{figure}
The basic process of generating test cases in our approach is as follows:

SmartUnit accepts the .c and .h files as its input. To deal with macros and make sure some external symbols can be introduced into the source file, we use \textit{libclang}\footnote{http://clang.llvm.org/doxygen/group\_\_CINDEX.html} as preprocessor to generate processed.c file. Then libclang is also used to parse the processed file to generate the AST (abstract syntax tree).

We establish the CFG (control flow graph) model based on the abstract syntax tree generated in the previous step, which consists control flow graph of the file being proceeded, in which type information of variables, expressions, functions and so on is stored to be used in further analysis. Each node in control flow graph represents a statement block in the source code. A sequential node, which contains exactly one incoming edge and one outgoing edge, contains no branch, meanwhile a branch node, which contains one incoming edge and more than one outgoing edge every of which shows a condition of a branch, is a statement block that contains conditional statements, such as if-else statement, while statement, switch statement \etc. 

\subsection{Executor Module}
Executor module consists of the memory model, executor, and searcher. This part mainly processes the CFG model given by former steps.

\subsubsection{Executor}
Executor executes the statement expressions in the current node and drives the searcher to select next edge to explore. The executor does not really execute the C statements, it actually transforms the C statement into blocks, declarations or expressions structures that are stored inside SmartUnit. The executor updates information in CFG model and adds constraints to a path, after gathering them from the node statement. After the executor reaches the end node, it collects all constraints on the path, and solves them by constraint solver such as Z3 prover.

\subsubsection{Searcher and Search Strategies}
To perform the search on control flow graph, we put forward a new search strategy, named flood-search policy. The algorithm is inspired by the situation that nodes and edges in CFG are an analogy for reservoirs and gates between reservoirs, with the starting point of the CFG as the flood point.

Algorithm.\ref{algo:search} is the description of the search algorithm.
Suppose the starting node \emph{n} is flooded, all the sides of the graph are reservoirs, all the nodes of the graph are gates, each gate have two states (open/closed). If there are one or more empty reservoirs (edge) in the current path, the path is considered a valuable path, we will save the current execution state and find the shortest path to the program exit as soon as possible to get the value of this path, which means that the new constraints will be collected. If all reachable 
paths of the current nodes or edges have no value (path have no unvisited edges), these nodes or edges have no value as well.

In our CFG model, each node in the graph represents a basic statement block, directed edges are used to represent jumps in the control flow. The branch edges of branch node record the branch condition and their result (true/false). Because the main goal of the search is to cover all branch edges in the graph, when encountering a branch node, flood-search policy forks a copy of current execution state, and adds the new execution state to open or close list, depending on the visit status of its branch.

If the input is G(edges, nodes), which is a CFG model. At the beginning, we push the state initialized by the start node into the open list, while the closed list is empty. Then the search starts to get execution states from the open list, and executes them by order, suppose the current execution state is \emph{s}. Every execution state in the open list is considered to be valuable, which means it may have new constraints, so flood-search will search the shortest way from the current executed node in \emph{s} to the exit node to keep this path, and make sure constraints in this path will be collected.

After the current execution state is executed, the next execution state of \emph{s} will be executed. If the current executed node in \emph{s} is a branch node and the node has more than one unvisited node, \emph{s} should be added to open list, because the unvisited branch of \emph{s} must be traversed. Even if \emph{s} has no unvisited branch, it still possibly has a succeed path unvisited, so \emph{s} should be stored in the close list, and prepared for further searching.

Compared with other graph searching algorithms such as BFS or DFS, flood-search fits well for CFG traverse, for flood-search trying to visit unvisited edges and nodes as early as possible, meanwhile, BFS or DFS may be caught in the loop.

\begin{algorithm2e}
\small
  \setcounter{AlgoLine}{0}
\caption{Flood-search for Control Flow Graph}\label{algo:search}
\DontPrintSemicolon
\newcommand\mycommfont[1]{\small\sffamily\textcolor{gray}{#1}}
\SetCommentSty{mycommfont}
% \KwInput{ \begin{tabularx}{.9\linewidth}{>{$}c<{$} X}
%     c_1,\ldots c_N  & the cut path
%   \end{tabularx}}

\KwIn{$G(edges,nodes)$: a control flow graph}

\BlankLine

$open$ $\gets$ \{State(Root($G$))\}, $close$ $\gets$ \{\}

\Repeat{$open$.size $=$ 0}
{
 SearchShortestToExit(Pop($open$));
 \;
 \If{$open$.size $=$ 0} {
  Discharge();
 }
}

\BlankLine

\textbf{Procedure} SearchShortestToExit(State $s$)

 \If{$s$ is on the end node of the graph}{
 \Return
 }
 $next\_state$ $\gets$ Next($s$);
 \;
 \If{$s$ has unvisited edge}{
 $open \gets open \cup \{s\}$\;
 }
 \ElseIf{$s$ has visited edge}{
 $close \gets close \cup \{s\}$\;
 }
 \Else{
 $close \gets close \cup \{s\}$\;
 \Return}
 SearchShortestToExit($next\_state$);
 \;
 \;
 
\textbf{Procedure} Discharge()
 \;
 \Repeat{$close$.size $=$ 0}
 {
  $open$ $\gets$ $open$ $\cup$ \{Next(Pop($close$))\}\;
 }

\end{algorithm2e}

\subsubsection{Memory model}
The memory model is the key module to track execution states and gather constraints, by simulating whole memory allocation.
Very basically, memory model stores all variables of basic types, such as int, char, including their names and values.
Dealing with complex types, such as the pointer, is a challenge for analysis tools. 
Our solution is below. For the array of basic types, in addition to memory space needed by the variable in the array, the total size of the array will also be stored, to perform plus/minus on pointers, and check if the pointer is out of memory bound. Furthermore, to deal with the member of the struct, union or enum, the total data structure and the start location in memory are needed to locate the variable by start location and the memory offset. 

\subsection{Cloud-based Testing Environment}
The SmartUnit Service contains all other features except the core analysis module, including web frontend UI, backend master process to handle web requests, worker process to perform analysis actions, database module to store test results.
The SmartUnit System architecture diagram is shown in Figure.~\ref{fig:web}.
\begin{figure}
    \includegraphics[width=0.3\textwidth]{Figs/web.pdf}
    \caption{The workflow of the cloud-based platform.}
    \label{fig:web}
\end{figure}
Web UI is designed to manage projects to be tested and get the results. Tested project is needed to be uploaded to the server after archived, and will be passed to master process for further operations.
The master process extracts the uploaded archive, creates a record in the database, and forks a worker process to call SmartUnit analysis engine to generate test cases for the project.

After SmartUnit finishes its analysis, worker process updates the status and saves generated in the database, then status in Web UI is also updated, after which users could download test cases in specific formats.
When the master process receives a request about specific test case, it will check if the test case is already prepared. If not, master process will generate a test case file according to test case data in the database and required file format. After finished, the test case archive is returned to the Web UI and could be reused in further downloading.

\subsection{Challenges and Solutions}
\subsubsection{Pointer}
The symbolizing  of the pointer variable is a big challenge, because the pointer operations need to access the real value of the pointer and the variable that pointer points to. The real value of the pointer is hard to access as it is regarded as a symbolic value that means we must maintain a pointer array of pointer owner to execute a pointer operation, and the length of this array may be infinite because the pointer execution could be everything. 

SmartUnit can support pointer operations, while a pointer memory must include the array memory of its owner which the pointer belongs to, the offset to address the position of the pointer, and some other marks such as null pointer mark. For the array of basic types, in addition to memory space needed by the variable in the array, the size of array will also be stored, to perform plus/minus operations on pointers, and check if pointer is out of memory bound.

\subsubsection{void*}
In most embedded C programs, (void*) is a special data type treated as a type that means nothing and used to transform data without data type. In Memory model, each pointer typed (void*) will be stored with its original type.
SmartUnit implements this by maintaining a void memory type and saves the alias of the memory in it. When executor comes to the (void*), it will create a voidmemory type, and record its type information to the aliased memory of the voidmemory. It will update the aliased memory when executing to the assignment of void*, and look up to its alias memory rather than voidmemory itself, so that we can get the type and memory information of the void* type.

\subsubsection{Complex data structure}
Complex data structures like struct, union or enum type are hard to handle, for they do not have a fixed length. To deal with the members of the struct, union or enum type, the total data structure and the start location in memory are needed to locate the variable by start location and the memory offset.

For a struct memory, the difficulty is to do operations related to the index. Thus, in addition to storing all variable declaration, the start and end memory location and relation between previous and next memory block are also needed to be stored.

==> results_and_analysis.tex <==
\section{results and analysis}
\textbf{RQ1: How about the performance of automated unit test generation framework SmartUnit in both commercial embedded software and open-source database software?}
For this question, we pushed the benchmarks to the SmartUnit testing platform, made it run automatically, and got the coverage from the web view.
Table~\ref{table:RQ1_coverage} shows the coverage information of the benchmarks. In Column \emph{Subject}, the items represent the name of the programs in our benchmark. The Column \emph{\#Test cases} represents the number of test cases 
generated by SmartUnit for the corresponding benchmark.
SmartUnit calculated coverage for each module individual because we separated PostgreSQL into the divided modules. Thus, we used PostgreSQL plus module names as the benchmark names in Table~\ref{table:RQ1_coverage}. 
The numbers in Statement Coverage, Branch Coverage, and MC/DC Coverage represent the number of functions in the corresponding range. The number of functions which achieve 100\% coverage is high lighted in gray.

In general, more than 90\% of functions in commercial embedded software achieve 100\% statement, branch, MC/DC coverage, 
more than 80\% of functions in SQLite achieve 100\% statement, branch, MC/DC coverage, and more than 60\% of functions in PostgreSQL achieve 100\% statement, branch, MC/DC coverage. 
As Table~\ref{table:RQ1_coverage} shows, most of the functions achieve 100\% statement, branch, MC/DC coverage.
Except for 100\% coverage, the number of functions is the even distribution in other coverage ranges. 

From the data, the conclusion is SmartUnit have a good performance on commercial embedded software and SQLite which is used in embedded systems.
The performance on PostgreSQL not as good as commercial embedded software and SQLite, but is also well enough.
It means SmartUnit is more suitable for embedded software and also have a well enough performance on common software.
However, there are also some functions not achieving 100\% of statement, branch, MC/DC coverage, 
what factors make SmartUnit not get 100\% coverage will be discussed in RQ2.

\begin{table*}
    \Huge
    \centering
    \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
    \resizebox{\textwidth}{!}{\begin{minipage}{\textwidth}
    \centering
    \caption{Performance of \textit{SmartUnit} on coverage.}
    \label{table:RQ1_coverage}
    \resizebox{\textwidth}{!}{% Resize table to fit within \linewidth horizontally
    \begin{tabular}{|c|c|ccccc|ccccc|ccccc|}
    \toprule
    \multicolumn{1}{|c|}{Subject} 
    &\multicolumn{1}{c|}{\#Test cases} 
    &\multicolumn{5}{c|}{Statement Coverage (\#Functions)} 
    &\multicolumn{5}{c|}{Branch Coverage (\#Functions)} 
    &\multicolumn{5}{c|}{MC/DC Coverage (\#Functions)} 
    \\

    &
    &0\%-10\% &10\%-50\% &50\%-90\% &90\%-100\% &100\% 
    &0\%-10\% &10\%-50\% &50\%-90\% &90\%-100\% &100\% 
    &0\%-10\% &10\%-50\% &50\%-90\% &90\%-100\% &100\% 

    \\ \hline
    \tabincell{c}{\emph{aerospace software}}
    & \tabincell{c}{712}
    %SC
    & \tabincell{c}{1}
    & \tabincell{c}{4}
    & \tabincell{c}{5}
    & \tabincell{c}{4}
    & \tabincell{c}{\cellcolor{gray!30}40}
    %BC
    & \tabincell{c}{1}
    & \tabincell{c}{4}
    & \tabincell{c}{5}
    & \tabincell{c}{3}
    & \tabincell{c}{\cellcolor{gray!30}40}
    %MC/DC
    & \tabincell{c}{3}
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}51}
    
    
    \\ \hline
    \tabincell{c}{\emph{automotive software}}
    & \tabincell{c}{3134}
    %SC
    & \tabincell{c}{1}
    & \tabincell{c}{3}
    & \tabincell{c}{9}
    & \tabincell{c}{2}
    & \tabincell{c}{\cellcolor{gray!30}315}
    %BC
    & \tabincell{c}{1}
    & \tabincell{c}{6}
    & \tabincell{c}{8}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}315}
    %MC/DC
    & \tabincell{c}{3}
    & \tabincell{c}{3}
    & \tabincell{c}{1}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}323}
    
    
    \\ \hline
    \tabincell{c}{\emph{subway signal software}}
    & \tabincell{c}{14848}
    %SC
    & \tabincell{c}{1}
    & \tabincell{c}{5}
    & \tabincell{c}{23}
    & \tabincell{c}{37}
    & \tabincell{c}{\cellcolor{gray!30}808}
    %BC
    & \tabincell{c}{1}
    & \tabincell{c}{5}
    & \tabincell{c}{35}
    & \tabincell{c}{33}
    & \tabincell{c}{\cellcolor{gray!30}800}
    %MC/DC
    & \tabincell{c}{7}
    & \tabincell{c}{5}
    & \tabincell{c}{9}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}853}
    
    
    \\ \hline
    \tabincell{c}{\emph{SQLite}}
    & \tabincell{c}{6814}
    %SC
    & \tabincell{c}{95}
    & \tabincell{c}{85}
    & \tabincell{c}{147}
    & \tabincell{c}{62}
    & \tabincell{c}{\cellcolor{gray!30}1657}
    %BC
    & \tabincell{c}{98}
    & \tabincell{c}{111}
    & \tabincell{c}{144}
    & \tabincell{c}{66}
    & \tabincell{c}{\cellcolor{gray!30}1627}
    %MC/DC
    & \tabincell{c}{146}
    & \tabincell{c}{68}
    & \tabincell{c}{140}
    & \tabincell{c}{8}
    & \tabincell{c}{\cellcolor{gray!30}1684}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL bootstrap}}
    & \tabincell{c}{27}
    %SC
    & \tabincell{c}{1}
    & \tabincell{c}{9}
    & \tabincell{c}{2}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}9}
    %BC
    & \tabincell{c}{1}
    & \tabincell{c}{11}
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}9}
    %MC/DC
    & \tabincell{c}{12}
    & \tabincell{c}{-}
    & \tabincell{c}{1}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}8}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL catalog}}
    & \tabincell{c}{1197}
    %SC
    & \tabincell{c}{10}
    & \tabincell{c}{91}
    & \tabincell{c}{131}
    & \tabincell{c}{7}
    & \tabincell{c}{\cellcolor{gray!30}186}
    %BC
    & \tabincell{c}{14}
    & \tabincell{c}{148}
    & \tabincell{c}{75}
    & \tabincell{c}{13}
    & \tabincell{c}{\cellcolor{gray!30}175}
    %MC/DC
    & \tabincell{c}{183}
    & \tabincell{c}{31}
    & \tabincell{c}{8}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}203}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL initdb}}
    & \tabincell{c}{312}
    %SC
    & \tabincell{c}{-}
    & \tabincell{c}{2}
    & \tabincell{c}{3}
    & \tabincell{c}{6}
    & \tabincell{c}{\cellcolor{gray!30}61}
    %BC
    & \tabincell{c}{-}
    & \tabincell{c}{4}
    & \tabincell{c}{10}
    & \tabincell{c}{11}
    & \tabincell{c}{\cellcolor{gray!30}49}
    %MC/DC
    & \tabincell{c}{2}
    & \tabincell{c}{-}
    & \tabincell{c}{9}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}61}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL pg\_dump}}
    & \tabincell{c}{1608}
    %SC
    & \tabincell{c}{16}
    & \tabincell{c}{27}
    & \tabincell{c}{60}
    & \tabincell{c}{25}
    & \tabincell{c}{\cellcolor{gray!30}378}
    %BC
    & \tabincell{c}{20}
    & \tabincell{c}{36}
    & \tabincell{c}{60}
    & \tabincell{c}{38}
    & \tabincell{c}{\cellcolor{gray!30}352}
    %MC/DC
    & \tabincell{c}{37}
    & \tabincell{c}{22}
    & \tabincell{c}{32}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}415}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL pg\_resetxlog}}
    & \tabincell{c}{65}
    %SC
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{2}
    & \tabincell{c}{1}
    & \tabincell{c}{\cellcolor{gray!30}8}
    %BC
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{2}
    & \tabincell{c}{1}
    & \tabincell{c}{\cellcolor{gray!30}8}
    %MC/DC
    & \tabincell{c}{-}
    & \tabincell{c}{1}
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}10}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL pg\_rewind}}
    & \tabincell{c}{245}
    %SC
    & \tabincell{c}{4}
    & \tabincell{c}{1}
    & \tabincell{c}{2}
    & \tabincell{c}{4}
    & \tabincell{c}{\cellcolor{gray!30}53}
    %BC
    & \tabincell{c}{4}
    & \tabincell{c}{1}
    & \tabincell{c}{2}
    & \tabincell{c}{5}
    & \tabincell{c}{\cellcolor{gray!30}52}
    %MC/DC
    & \tabincell{c}{4}
    & \tabincell{c}{-}
    & \tabincell{c}{4}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}56}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL pg\_upgrade}}
    & \tabincell{c}{305}
    %SC
    & \tabincell{c}{6}
    & \tabincell{c}{3}
    & \tabincell{c}{5}
    & \tabincell{c}{5}
    & \tabincell{c}{\cellcolor{gray!30}81}
    %BC
    & \tabincell{c}{6}
    & \tabincell{c}{4}
    & \tabincell{c}{4}
    & \tabincell{c}{9}
    & \tabincell{c}{\cellcolor{gray!30}77}
    %MC/DC
    & \tabincell{c}{8}
    & \tabincell{c}{2}
    & \tabincell{c}{9}
    & \tabincell{c}{1}
    & \tabincell{c}{\cellcolor{gray!30}80}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL pg\_xlogdump}}
    & \tabincell{c}{67}
    %SC
    & \tabincell{c}{3}
    & \tabincell{c}{2}
    & \tabincell{c}{2}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}11}
    %BC
    & \tabincell{c}{3}
    & \tabincell{c}{2}
    & \tabincell{c}{3}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}10}
    %MC/DC
    & \tabincell{c}{3}
    & \tabincell{c}{1}
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}14}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL pgtz}}
    & \tabincell{c}{9112}
    %SC
    & \tabincell{c}{587}
    & \tabincell{c}{595}
    & \tabincell{c}{704}
    & \tabincell{c}{68}
    & \tabincell{c}{\cellcolor{gray!30}2465}
    %BC
    & \tabincell{c}{617}
    & \tabincell{c}{872}
    & \tabincell{c}{475}
    & \tabincell{c}{51}
    & \tabincell{c}{\cellcolor{gray!30}2404}
    %MC/DC
    & \tabincell{c}{1393}
    & \tabincell{c}{233}
    & \tabincell{c}{139}
    & \tabincell{c}{8}
    & \tabincell{c}{\cellcolor{gray!30}2646}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL psql}}
    & \tabincell{c}{1378}
    %SC
    & \tabincell{c}{3}
    & \tabincell{c}{13}
    & \tabincell{c}{18}
    & \tabincell{c}{14}
    & \tabincell{c}{\cellcolor{gray!30}380}
    %BC
    & \tabincell{c}{3}
    & \tabincell{c}{15}
    & \tabincell{c}{19}
    & \tabincell{c}{18}
    & \tabincell{c}{\cellcolor{gray!30}373}
    %MC/DC
    & \tabincell{c}{10}
    & \tabincell{c}{12}
    & \tabincell{c}{27}
    & \tabincell{c}{2}
    & \tabincell{c}{\cellcolor{gray!30}377}
    
    
    \\ \hline
    \tabincell{c}{\emph{PostgreSQL scripts1}}
    & \tabincell{c}{189}
    %SC
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{7}
    & \tabincell{c}{4}
    & \tabincell{c}{\cellcolor{gray!30}30}
    %BC
    & \tabincell{c}{-}
    & \tabincell{c}{-}
    & \tabincell{c}{7}
    & \tabincell{c}{6}
    & \tabincell{c}{\cellcolor{gray!30}28}
    %MC/DC
    & \tabincell{c}{-}
    & \tabincell{c}{2}
    & \tabincell{c}{6}
    & \tabincell{c}{-}
    & \tabincell{c}{\cellcolor{gray!30}33}
    \\
    
\bottomrule
\end{tabular}}
\end{minipage}}
\end{table*}

\lstset{
    frame=tb,
    language=C,
    aboveskip=3mm,
    belowskip=3mm,
    showstringspaces=false,
    columns=flexible,
    basicstyle={\small\ttfamily},
    breaklines=true,
    breakatwhitespace=true,
    tabsize=3,
    basicstyle=\footnotesize\ttfamily
}

\textbf{RQ2: What factors make dynamic symbolic execution get low coverage?}
In Table.~\ref{table:RQ1_coverage}, although SmartUnit has the high statement, branch, and MC/DC coverage,
there are some function units has a low coverage (\eg 0\%-10\%).
We found the low coverage functions, read the source code and analysis manually to find out why SmartUnit
get the low coverage in these functions. We categorized the main reasons as follows:

\textbf{Environment variable and Environment function:} 
In the benchmarks, there is a variety of environment variable and environment function in the code. 
For example, the current time is an environment variable, it comes from the system and is difficult to be symbolized.
Environment function are usually standard library calls, such as \textit{sizeof()}. 
Listing.~\ref{lst:sizeof} is an example from PostgreSQL. 
It is difficult to covert the condition in line 4 to a constraint, because symbolic execution engine is hard to comprehend the semantic of the environment functions. Therefore, the coverage can not achieve 100\% in this situation.
\begin{lstlisting}[caption={An example of environment function.},label={lst:sizeof},language=C]
static void handle_sigint(SIGNAL_ARGS)
{
        ...
        if (PQcancel(cancelConn, errbuf, sizeof(errbuf)))
        {
            CancelRequested = true;
            fprintf(stderr, _("Cancel request sent\n"));
        }
        else
            fprintf(stderr, _("Could not send cancel request: %s"), errbuf);
        ...
}
\end{lstlisting}


\textbf{Complex operation:} Although we have a solution to deal with the variable pointer, the complex operation is difficult to deal with.
Listing.~\ref{lst:complex} comes from SQLite. There is a complex pointer operation in line 4 which combines variable pointers and function pointers. 
Due to the limit of the memory model, it can not handle these complex operations.
Execution will be terminated by this kind of statement and get a low coverage.
\begin{lstlisting}[caption={An example of environment function.},label={lst:complex},language=C]
static void callFinaliser(sqlite3 *db, int offset){
 ...
 int (*x)(sqlite3_vtab *);
 x = *(int (**)(sqlite3_vtab *))((char *)p->pModule + offset);
 if( x ) x(p);
 ...
}
\end{lstlisting}

\textbf{limitation of SMT solver:} In SmartUnit, Z3 Solver is the main SMT solver to solve the constraint. 
Although Z3 is one of the best SMT solvers, it still has some limitation. Here is an example.
\textit{y != 0 \&\& (((x-1) * y) \% y) == 1} is a constraint collected by SmartUnit in the commercial software. 
Although it is a legal constraint and there is no divided by zero faults, the Z3 solver can not deal with it.
The Z3 solver developer said that Z3 could not deal with nonlinear constraints, such as this constraint.
It is the common reason for getting the low coverage.
Thus the coverage of symbolic execution is sometimes affected by the SMT solver.

\textbf{RQ3: Can SmartUnit find the potential runtime exception in real-world software?}
From RQ1, we found that SmartUnit has a high coverage on the real world software. 
During the execution, there are also some of the potential runtime exceptions in this software.
Except the factors discussed in RQ2, we found more than 5,000 number of test cases with runtime exceptions. Due to the time limit, we have not checked every test case manually, we sampled from the test cases to analysis the runtime exceptions. Generally, we divided the runtime exceptions found by SmartUnit into three categories: 
array index out of bounds, fixed memory address and divided by zero. 

\textbf{Array index out of bounds:} As the introduction in Section 3, SmartUnit use memory model to simulate whole memory allocation.
if there is an array index out of bounds, SmartUnit will throw a runtime exception. 
Listing.~\ref{lst:array} is an example comes from SQLite. 
Obviously, in this function, there is an out of bounds runtime exception in line 10, when \emph{i \textless argc}. 
Although the caller of this function ensure \emph{i \textless= argc} in SQLite, 
it has a potential runtime exceptions if other callers not ensure \emph{i \textless= argc}.
There is even no precondition in the comment.
It is quite serious if a programmer wants to call it, but doesn't know the precondition.
We have found much of runtime exceptions in this category from all of the benchmarks.

\begin{lstlisting}[caption={An example of array index out of bounds.},label={lst:array},language=C]
/*
** Get the argument to an --option.  Throw an error and die if 
** no argument is available.
*/
static char *cmdline_option_value(int argc, char **argv, int i) {
    if (i == argc) {
        utf8_printf(stderr, "%s: Error: missing argument to %s\n", argv[0], argv[argc - 1]);
        exit(1);
    }
    return argv[i];
}
\end{lstlisting}

\textbf{Fixed memory address:} Fixed memory address is a problem in dealing with the variable pointer. 
In the embedded system, there are many pointer operations with the fixed memory address. 
It is hard for memory model to simulate a fixed memory address.
For example, the operations like (*0X00000052) or (* (symbolic variable + 12)) will cause runtime exceptions.
It usually gets \textit{NULL} when referring from a fixed memory address.
Thus symbolic execution will throw runtime exception with fixed memory address operations.


\textbf{Divided by zero:} Divided by zero is also a common runtime exception in the benchmarks. 
It usually appears in numerical calculation of program. 
SmartUnit will generate boundary value to check if the program exists divided by zero runtime exception.
We select a brief example from SQLite to discuss this runtime exception. 
Listing.~\ref{lst:zero} is the function which has the potential runtime exception in line 19.
When \emph{nUsable == 4}, the expression \emph{(nTotal - nMinLocal) \% (nUsable - 4)} will throw a divided by zero runtime exception.
we read the source code manually and found that it is difficult to comfirm whether \emph{nUsable} could be 4 or not.
The comment of the function does not contain the precondition of \emph{nUsable}.
It's horrible if the programmer who calls this function in a new function and do not know the implicit prediction.

\begin{lstlisting}[caption={An example of divided by zero.},label={lst:zero},language=C]
static void getLocalPayload(
  int nUsable,                    /* Usable bytes per page */
  u8 flags,                       /* Page flags */
  int nTotal,                     /* Total record (payload) size */
  int *pnLocal                    /* OUT: Bytes stored locally */
){
  int nLocal;
  int nMinLocal;
  int nMaxLocal;
 
  if( flags==0x0D ){              /* Table leaf node */
    nMinLocal = (nUsable - 12) * 32 / 255 - 23;
    nMaxLocal = nUsable - 35;
  }else{                          /* Index interior and leaf nodes */
    nMinLocal = (nUsable - 12) * 32 / 255 - 23;
    nMaxLocal = (nUsable - 12) * 64 / 255 - 23;
  }

  nLocal = nMinLocal + (nTotal - nMinLocal) % (nUsable - 4);
  if( nLocal>nMaxLocal ) nLocal = nMinLocal;
  *pnLocal = nLocal;
}
\end{lstlisting}

In summary, SmartUnit could find the potential runtime exceptions in real-world software. We categorized and analyzed the potential runtime exceptions. 
Most of these potential runtime exceptions existed, due to there is no protection for input values.
At the same time, there is no clear precondition specification for the functions.
Although there are protection codes in the caller of the function, the potential runtime exceptions may cause the real faults in real-world software.



\textbf{RQ4: What is the difference between automatically generated test cases and manually written test cases?}
In RQ4, we compare automatically generated test cases and manually written test cases in the following aspect: time, cost and quality.

\textbf{Time \& Cost:} Table~\ref{table:RQ4_time} shows the test set generated time for each benchmark. 
The column \textit{Subject} list all of the benchmark we used.
As Table~\ref{table:RQ1_coverage}, we separate PostgreSQL into the individual module, and name with PostgreSQL plus module name.
The second column \textit{\# Functions} represents the number of functions in the benchmark.
The column \textit{Time} means the test set generated time for the corresponding benchmark.
The column \textit{Average} represents the average test set generated time for the corresponding benchmark per function, 
in other words, it means the average time of SmartUnit generates test set for a function.
Deserve to be mentioned, we use \textit{Total\# Function} and \textit{Total Time} to calculate \textit{Total Average}.

In Table~\ref{table:RQ4_time}, it is obvious that the average time ranges from 1s to 7s and total average time is 3.77s for all of the benchmarks.
It means that SmartUnit spends nearly 4s to generate test cases for a function, 
and in the best situation, more than 90\% of the functions can achieve 100\% statement, branch, and MC/DC coverage.
How about the test engineer? In our survey from companies, a trained test engineer can product test case for 5-8 functions per day. 
Thus using automated unit test generation framework can cost less time than employing test engineers. 

The main cost of automatically generated test cases and manually written test cases are both the salary paid for the employee. We assume a
developer costs twice salary higher than a test engineer. SmartUnit has cost 24 man-month to release. For manually testing, 
a test engineer could write the test case for about 160 functions per month. Thus 24 man-month cost could support test engineers write about 8,000 functions. 
In summary, if you have a large number of function units(\eg more than 10,000), automatically generated test cases are cheaper.
On the contrary, manual test cases are cheaper for the little scale of projects. 

\textbf{Quality:} From RQ1, we have the conclusion that more than 90\% of functions in commercial embedded software can achieve 100\% statement, branch and MC/DC coverage; more than 80\% of functions in SQLite achieve 100\% coverage, and more than 60\% of functions in PostgreSQL achieve 100\% coverage. According to our survey in the companies, the test engineers need to achieve 100\% coverage for each function. If we use coverage as a quality indicator, automatically generated test case has overwhelming superiority on cost and time though manual test case has higher coverage in some cases. Meanwhile, the automatically generated test cases could find runtime exception in time. 

\begin{table}[!t]
\footnotesize
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%% increase table row spacing, adjust to taste
\renewcommand{\arraystretch}{1}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
\caption{Test set generated time for each benckmark.}
\label{table:RQ4_time}
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
\begin{tabular}{|c||c|c|c|}
\hline
Subject &\# Functions &Time (s) &Average (s/func) \\
\hline
\hline
aerospace software &54 &318 &6\\
automotive software &330 &329 &1\\
subway signal software &874 &2,476 &3\\
SQLite &2046 &13,482 &6\\
PostgreSQL bootstrap &21 &48 &2\\
PostgreSQL catalog &425 &1,350 &3\\
PostgreSQL initdb &72 &548 &7\\
PostgreSQL pg\_dump &506 &3,428 &7\\
PostgreSQL pg\_resetxlog &11 &71 &6\\
PostgreSQL pg\_rewind &64 &352 &5\\
PostgreSQL pg\_upgrade &100 &465 &5\\
PostgreSQL pg\_xlogdump &18 &130 &7\\
PostgreSQL pgtz &4419 &10,478 &2\\
PostgreSQL psql &428 &1,676 &4\\
PostgreSQL scripts1 &41 &311 &7\\


\hline
\hline
Total &9,409 &35,462 &3.77\\
\hline
\end{tabular}
\end{table}

\textbf{Discussion}

Traditional automated unit testing tools focus on the automated random testing, \eg, test cases are randomly derived as the input to invoke the program code under test. Although the random test data generation algorithm is quite easy to be implemented, it is obviously that the expected coverage criteria (e.g., the branch and the statement coverage) cannot be guaranteed. The DART (Directed Automated Random Testing) is a classical unit testing tool that supports the directed random test data generation~\cite{godefroid2005dart}. One unique characteristic of the DART is its complete automation for unit testing. Since its underlying approach is random testing, the DART focuses on detecting standard errors such as program crashes, assertion violations, and non-termination while it is not deliberately designed for certain coverage criteria requested by the industrial standards. Our SmartUnit framework can handle the automated testing and support various coverage criteria of the industrial standards.

   PEX is a famous unit testing tool that automatically generates test suites with high code coverage~\cite{tillmann2008pex}. It is a Visual Studio add-in for testing .NET Framework applications. In practice, the PEX tool is adapted to testing the C\# code. Similarly the IntelliTest\footnote{https://msdn.microsoft.com/en-us/library/dn823749.aspx} also automatically generates test data for the unit test of C\#. The basic idea of the IntelliTest is to generate test data to execute each statement of the target code and then analyze the coverage of the conditional branch. The Microsoft Security Risk Detection is a unique fuzz testing service for finding security critical bugs in software. These three tools significantly improve the unit testing in bug detection and time efficiency. However, since these tools are designed as general solutions for unit testing, it cannot be directly applied in the domain of real-time control software testing. They fall short in supporting the unit testing of the control software since some unique features such as the high coverage request of particular criteria requested by the industrial standards have not been deliberately considered. The SmartUnit framework focuses on the request of current industry standards and offers a completely automated solution for the unit testing of the real-time software.
   
Although there is a plug-in of Testbed called LDRA TBrun\footnote{http://ldra.com/industrial-energy/products/tbrun/} which can automatically generate driver program and test harness without manual script,
SmartUnit is quite different from it.
LDRA TBrun uses data dictionary to generate the test cases, it combines several values in the data dictionary, 
usually considering up bound and low bound of variables. 
This strategy is not able to deal with memory calculation, while SmartUnit can easily catch memory change constraints by DSE.
LDRA TBrun generates unit test suite based-on boundary value (\eg, maximum value, minimum value, median value, \etc),
while SmartUnit is a coverage-driven tool, it can satisfy statement, branch, MC/DC coverage criteria from industrial requirements.
SmartUnit can avoid repetitive test cases, while LDRA TBrun has many repetitive test cases in its test set.
LDRA TBrun can not give the expectative output value for each test case, 
but SmartUnit can expect output value by executing test cases automatically after generation.
SmartUnit can not only generate the test cases for function parameters and global variables which support in LDRA TBrun,
it can also generate the test cases for instrument function parameters and instrument function return value. 
In summary, LDRA TBrun is suitable for critical testing and robustness testing,
while SmartUnit is suitable for coverage-driven testing.
